Towards Efficient Data-Centric Robust Machine Learning with Noise-based Augmentation

The data-centric machine learning aims to find effective ways to build appropriate datasets which can improve the performance of AI models. In this paper, we mainly focus on designing an efficient data-centric scheme to improve robustness for models towards unforeseen malicious inputs in the black-box test settings. Specifically, we introduce a noised-based data augmentation method which is composed of Gaussian Noise, Salt-and-Pepper noise, and the PGD adversarial perturbations. The proposed method is built on lightweight algorithms and proved highly effective based on comprehensive evaluations, showing good efficiency on computation cost and robustness enhancement. In addition, we share our insights about the data-centric robust machine learning gained from our experiments.

==> Sections/2-related_works.tex <==
\section{Related Works}\label{related}

To build a model with good robustness and high accuracy is a big topic and involves many research findings from different fields.

==> Sections/alg-1.tex <==
\begin{algorithm}[t]
\caption{SGD with CosineAnnealingWarmRestarts}
\label{alg}
\textbf{Input}: Parameters $\theta_t$; minimum learning rate $\gamma_{min}$; maximum learning rate $\gamma_{max}$; loss function $\Phi$; weight decay $\lambda$; momentum $\mu$; dampening $\tau$; the number of epochs since the last restart $T_{cur}$; the number of epochs between two warm restarts $T$.\\
\textbf{Output}: Parameters $\theta_{t+1}$.
\begin{algorithmic}[1] 
\STATE \textit{CosineAnnealingWarmRestarts Schedule.}
\IF{$T_{cur} == T$}
\STATE $\gamma = \gamma_{min}$;
\ELSIF{$T_{cur} == 0$}
\STATE $\gamma = \gamma_{max}$;
\ELSE
\STATE $\gamma = \gamma_{min} + \frac{1}{2}(\gamma_{max} - \gamma_{min})(1 + \cos{(\frac{T_{cur}}{T}\pi)})$;
\ENDIF
\STATE \textit{Stochastic Gradient Descent.}
\STATE $g_{t+1} \gets \nabla_{\theta}\Phi(\theta_{t})$
\STATE $g_{t+1} \gets g_{t+1} + \lambda\theta_{t}$
\STATE $g_{t+1} \gets \mu g_{t} + (1 - \tau)g_{t+1}$
\STATE $\theta_{t+1} \gets \theta_{t} - \gamma g_{t+1}$
\RETURN $\theta_{t+1}$
\end{algorithmic}
\end{algorithm}
